Lippmann Photography: A Signal Processing Perspective

Lippmann (or interferential) photography is the first and only analog photography method that can capture the full color spectrum of a scene in a single take. This technique, invented more than a hundred years ago, records the colors by creating interference patterns inside the photosensitive plate. Lippmann photography provides a great opportunity to demonstrate several fundamental concepts in signal processing. Conversely, a signal processing perspective enables us to shed new light on the technique. In our previous work, we analyzed the spectra of historical Lippmann plates using our own mathematical model. In this paper, we provide the derivation of this model and validate it experimentally. We highlight new behaviors whose explanations were ignored by physicists to date. In particular, we show that the spectra generated by Lippmann plates are in fact distorted versions of the original spectra. We also show that these distortions are influenced by the thickness of the plate and the reflection coefficient of the reflective medium used in the capture of the photographs. We verify our model with extensive experiments on our own Lippmann photographs.

==> sections/bios.tex <==
% !TeX spellcheck = en_US

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_photos/GillesBaechler.jpeg}}]{Gilles Baechler}
received his B.Sc. and his M.Sc. from EPFL in 2009 and 2012. In September 2018, he obtained his PhD degree in Computer and Communication Sciences at the  Audiovisual Communications Laboratory (LCAV) at EPFL, under the supervision of Prof. Martin Vetterli and Dr. Adam Scholefield.
In 2008 and 2009, he did a 1-year exchange in the Electrical and Computer Engineering department at Carnegie Mellon University in Pittsburgh, PA.
In 2010, he did an internship at the Cryptography and Security group at Bell Labs, Murray Hill, NJ. In 2012, he did his Master Thesis at Qualcomm, San Diego, CA in the Office of the Chief Scientist, where he worked on finite rate of innovation (FRI) sampling and ECG compression. In 2013, he worked at Morphean, providing intelligent solutions for detecting various events on video surveillance streams. In 2017, he did an internship as a software engineer at Google Zurich, working on a platform to automate threat detection.
His research interests include sparse sampling, image processing, computer vision and machine learning. Since 2018, he has been working at Google Research in Zurich, where he develops machine learning solutions for understanding graphical user interfaces.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_photos/MichalinaPacholska.jpg}}]{Michalina Pacholska}
received her B.Sc. and her M.Sc. in Mathematics from University of Warsaw in, respectively, 2014 and 2016. She holds a PhD in Computer Science from EPFL (Switzerland) where she worked on problems related to sampling theory, localization and Fourier optics. In 2018 she interned at Deepmind where she worked on the early stages of AlphaFold, leveraging deep-learning to solve the protein folding problem. Now Michalina leads research on the intersection of reinforcement learning with programme synthesis for social behavioural modelling at Improbable.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_photos/ArnaudLatty.jpg}}]{Arnaud Latty}
 received the M.S. degree in physics from École Polytechnique Fédérale de Lausanne (EPFL), Lausanne, Switzerland, in 2016, and the Teaching Diploma from ETH Zurich, Zurich, Switzerland, in 2020. Since 2017, he works as a scientific assistant with the Audiovisual Communications Laboratory, EPFL, and is increasingly hired as a secondary school teacher. His research interests include acoustics, optics (in particular hyperspectral recording), and didactics of physics.

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_photos/AdamScholefield.jpeg}}]{Adam Scholefield}
received the M.Eng. degree in electrical and electronic engineering and the Ph.D. degree from Imperial College London, London, U.K., in 2007 and 2013, respectively. He was a Postdoctoral Researcher with the Audiovisual Communications Laboratory, EPFL, Lausanne, Switzerland from 2014 to 2021. He represented Team GB in the 2012 Olympics and in 2020 he combined his sporting and technical interests by launching the startup We Play Sport SA, where he is currently co-founder and CTO.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_photos/vetterli_bio.eps}}]{Martin Vetterli}
     received the EE degree from ETHZ in 1981, the MS from Stanford University in 1982, and the Doctorate from EPFL in 1986. He was an Assistant/Associate  Professor in EE at Columbia University, and then an Associate/Full Professor in EECS at the UC Berkeley. In 1995, he joined the EPFL as a Full Professor. From 2004 to 2011 he was VP of EPFL for international affairs, and from 2011 to 2012, he was the Dean of IC. From 2013 to 2016 he was President of the Swiss NSF and since January 2017, he is President of EPFL. He works in the areas of electrical engineering, computer sciences and applied mathematics and this led to about 170 journals papers, as well as about 30 patents that led to technology transfer to high-tech companies and the creation of several start-ups. He is also the co-author of three textbooks.  His prizes include best paper awards from EURASIP in 1984 and of the IEEE Signal Processing Society in 1991, 1996 and 2006, the Swiss National Latsis Prize in 1996, the SPIE Presidential award in 1999, the IEEE SP Technical Achievement Award in 2001 and the IEEE SP Society Award in 2010 and the IEEE Jack S. Kilby Signal Processing Medal in 2017. He is a Fellow of IEEE, of ACM, ISI highly cited researcher and a foreign member of the NAE.
\end{IEEEbiography}

\vfill
